Self-supervised Auxiliary Learning for Graph Neural Networks via Meta-Learning

In recent years, graph neural networks (GNNs) have been widely adopted in the representation learning of graph-structured data and provided state-of-the-art performance in various applications such as link prediction, node classification, and recommendation. Motivated by recent advances of self-supervision for representation learning in natural language processing and computer vision, self-supervised learning has been recently studied to leverage unlabeled graph-structured data. However, employing self-supervision tasks as auxiliary tasks to assist a primary task has been less explored in the literature on graphs. In this paper, we propose a novel self-supervised auxiliary learning framework to effectively learn graph neural networks. Moreover, this work is the first study showing that a meta-path prediction is beneficial as a self-supervised auxiliary task for heterogeneous graphs. Our method is learning to learn a primary task with various auxiliary tasks to improve generalization performance. The proposed method identifies an effective combination of auxiliary tasks and automatically balances them to improve the primary task. Our methods can be applied to any graph neural network in a plug-in manner without manual labeling or additional data. Also, it can be extended to any other auxiliary tasks. Our experiments demonstrate that the proposed method consistently improves the performance of node classification and link prediction.

==> Figures_tex/fig_meta.tex <==
\begin{figure}][!htbp]
  \includegraphics[width=0.5\textwidth]{Figures/metapath.png}
\end{figure}

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Sections/4_6_Task_Selection.tex <==
\subsection{Task selection results}
Our proposed methods identify useful auxiliary tasks and balance them with the primary task. 
In other words, the loss functions for tasks are differentially adjusted by the weighting function learned by SELAR+HintNet. 
To analyze the weights of the tasks, we calculate the average of the task-specific weighted loss. 
Table. \ref{tab:MP} shows tasks in descending order of the task weights. `user-item-actor-item' has the largest weight followed by `user-item' (primary task), `user-item-appearing.in.film-item', `user-item-instruments-item', `user-item-user-item' and `user-item-artist.origin-item' on the Last-FM. 
It indicates that the preference of a given user is closely related to other items connected by an actor, e.g., specific edge type `film.actor.film' in the knowledge graph. 
Moreover, our method focuses on `user-item' interaction for the primary task.
On the Book-Crossing data, our method has more attention to `user-item' for the primary task and `user-item-literary.series-item-user' which means that users who like a series book have similar preferences. 


==> Sections/BroaderImpact.tex <==
\section*{Broader Impact}
We thank NeurIPS2020 for this opportunity to revisit the broader impact of our work and the potential societal consequence of machine learning researches. Our work is a general learning method to benefit from auxiliary tasks. One interesting finding is that meta-path prediction can be an effective self-supervised task to learn more power representation of heterogeneous graphs.  Nowadays, people use social media (e.g., Facebook, Twitter, etc.) on a daily basis.  Also, people watch movies and TV-shows online and purchase products on Amazon. All this information can be represented as heterogeneous graphs. We believe that our meta-path auxiliary tasks will benefit the customers with improved services. 
For instance, more accurate recommender systems will save customers' time and provide more relevant contents and products.  We believe that there is no direct negative consequence of this research. We proposed how to train models with auxiliary tasks. We did not make any algorithms for specific applications. So, no one will be put at a disadvantage from our work. No direct negative consequence of a failure of the system is expected. We used four datasets Last-FM, Book-Crossing, ACM, and IMDB. They may not represent all the population on the earth but our experiments did not leverage any biases in the datasets. We believe that our method will be as effective as we reported in the paper on different datasets from different populations.


==> Sections/memo.tex <==
\emph{\textbf{Auxiliary tasks. }}
To design the auxiliary task, we define the self-supervised learning tasks via generating the meta-path labels.
We generate directly multiple meta-path prediction labels by matrix multiplication of adjacency matrices represented each different relation. e.g., "user-item-user", "item-entity-item" and "user-item-entity-item", etc. 
Our auxiliary tasks are the link prediction for generated meta-path labels.
The primary task benefit from auxiliary tasks by predicting meta-paths which can capture diverse semantic information. 
We evaluate the benefits of the self-supervised auxiliary learning by predicting generated meta-path labels.
 Last-FM and Book-Crossing have 60 and 25 entity relations as shown in Table. \ref{tab:node}. We randomly select 5 types of meta-paths which have the path length is less than 4. The selected meta-path types in Last-FM are 'user-musician-user-musician', 'user-musician-artist.origin-musician', 'user-musician-person.or.entity.appearing.in.film-musician', 'user-musician-actor.film-musician' and 'user-musician-musician.instruments.played-musician'.
For instance, 'user-musician-artist.origin-musician' means that it has a meaningful relation among musicians who are the same place of birth. We infer that 'user-musician-musician.instruments.played-musician' is a given user will be interested in artists playing with same instruments .
In Book-Crossing, 'user-book-user', 'book-user-book', 'user-book-user-book', 'book-genre-book' and 'user-item-written.work.literary.series-book-user' are selected. 'book-genre-book' means that books of the same genre are related. A given user who likes a book series has a meaning that he will like some book series. For link prediction, the primary task, which is performed with the auxiliary task predicting meta-paths, is learned by reflecting the meaning of multiple meta-path.


\emph{\textbf{The number of Auxiliary Tasks.}}
We can use various numbers of meta-paths by varying their node and edge compositions for auxiliary tasks. Considering that a meta-path characterizes heterogeneous relations, we hypothesize the number of meta-paths influences the effects to assist the primary task because the the composition of meta-path relates to the difficulty of auxiliary tasks. Table~\ref{tab:abl_length} presents the results of our model for link prediction as the number of meta-paths used for auxiliary tasks increases. For verify the explicit effects of the meta-path number compared to Vanilla, we do not employ hint network. As shown in Table~\ref{tab:abl_length}, using meta-paths consistently improves the link prediction performance as on average 2.2\% and 3.3\% on Last-FM and Book-Crossing datasets for all base GNNs and their number. In particular, employing 3 meta-paths leads to the largest improvement on both datasets. Note that we can get more than 4\% of performance gain with auxiliary tasks of more than 2 meta-paths on Book-Crossing. We conjecture larger that a task that is moderately difficult rather than too easy one helps with generalization performance. With respect to base GNNs, we find that GIN most remarkably benefits from our auxiliary learning with meta-paths. 


% out both explicit weighting function and auxiliary tasks; \textbf{w/o meta-path}, learning a primary task only with the weighting function; \textbf{w/ meta-path}, training with multiple auxiliary tasks; \textbf{Selar}, learning to learn the primary task by auxiliary tasks; \textbf{Selar+Hint}, training with hint network by predicting meta-path as auxiliary tasks;  \\

% \subsection{Ablation Study}
% To further investigate the effects of Selar, we perform ablation study on two main components such as meta-path length and usages of meta cross-validation

% \input{Tables_tex/tab_num_metapath}


%
%\begin{table}[h]
%  \centering
%  \caption{The results of $AUC$ for link prediction}
%  \label{tab:link prediction}
%  \begin{tabular}{c|c|cc|ccc}
%    \toprule
%    & & & & \multicolumn{3}{c}{Ours} \\
%    \hline
%    Dataset & Basemodel & Vanilla & w/o meta-path & w/ meta-path & Selar & Selar+Hint \\
%    \toprule
%    \multirow{4}{*}{Music} & GCN & 0.7898 & 0.785 & 0.8135 & %\textbf{0.8163} & 0.8162 \\
%    & GAT & 0.809 & 0.81 & 0.8184 & 0.8319 & \textbf{0.8349} \\
%    & GIN & 0.7895 & 0.8081 & \textbf{0.8304} & 0.8211 & 0.8255 \\
%    & SGC & 0.7725 & 0.7759 & 0.7801 & 0.7803 & \textbf{0.7857} \\
%    \midrule
%    \multirow{4}{*}{Book} & GCN & 0.6918 & 0.6967 & 0.697 & \textbf{0.7081} & 0.7075 \\
%    & GAT & 0.6704 & 0.6759 & 0.7026 & 0.7136 & \textbf{0.7247} \\
%    & GIN & 0.6782 & 0.6968 & 0.7442 & 0.7554 & \textbf{0.7587} \\
%    & SGC & 0.6781 & 0.6732 & 0.6933 & \textbf{0.707} & 0.7039 \\

%    \toprule
%  \end{tabular}
%\end{table}








%\begin{table}[h]
%  \caption{Raw}
%  \label{sample-table}
%  \centering
%  \begin{tabular}{c|c|cccccc|c}
%    \toprule
%    & & Hint network & Vanilla & w/o meta-path & 1 meta-path & 3 meta-path & 5 meta-path & w/o MW \\
%    \midrule
%    & GCN & w/o & 0.7898 & 0.785 & 0.8071 & 0.825 & 0.8163 & 0.8135\\
%    & & w/ & - & - & 0.8067 & \textbf{0.8293} & 0.8162 & - \\
%    & GAT & w/o & 0.809 & 0.81 & 0.8226 & 0.8342 & 0.8319 & 0.8184 \\
%    & & w/ &- & - & 0.823 & 0.823 & \textbf{0.8349} & -\\
%    Music & & & & &&&&\\
%    & GIN & w/o & 0.7895 & 0.8081 & 0.8205 & 0.8208 & 0.8211 & \textbf{0.8304} \\
%    & & w/ & - &- & 0.8107 & 0.8146 & 0.8255 & - \\
%    & SGC & w/o & 0.7725 & 0.7759 & 0.7819 & 0.7818 & 0.7803 & 0.7801\\
%    & & w/ &- &-& 0.7844 & \textbf{0.791} &0.7857 & -\\
%    \midrule
%    & GCN & w/o & 0.6918 & 0.6967 & 0.7074 & \textbf{0.7156} & 0.7081 & 0.697\\
%    & & w/ & -&-&0.7037&0.7103&0.7075 & -   \\
%    & GAT & w/o & 0.6704 & 0.6759 & 0.6818 & 0.7169 & 0.7136 & 0.7026\\
%    & & w/ & -&-&0.6894 & \textbf{0.7344} & 0.7247&-\\
%    Book & & & & &&&&\\
%    & GIN & w/o &0.6782 & 0.6968 & 0.6944 & 0.7528 & 0.7554 & 0.7442\\
%    & & w/ & -&-&0.6925 & 0.7551 & \textbf{0.7587} & -\\
%    & SGC & w/o &  0.6781 & 0.6732 & 0.6864 & \textbf{0.7159} & 0.707 & 0.6933\\
%    & & w/ & -&-&0.6857 & 0.7128 & 0.7039 & -\\
    
%    \bottomrule
%  \end{tabular}
%\end{table}


% optimizer - Adam
% embedding dimension - 64 for node classifications
% number of layers are two for all models in node classification tasks.
% For each model, hyper parameters such as learning rate and weight decay are tuned for having best performance using validation datasets.
% \begin{table}[h]
%   \centering
%   \caption{$AUC$ of comparable methods with four base GNN models for link prediction}
%   \label{tab:link prediction}
%   \begin{tabular}{c|c|cc|ccc}
%     %\toprule
%     \hline\hline
%     % \multirow{2}*{Dataset}&\multirow{2}*{Base GNNs}&\multirow{2}*{Vanilla}&\multirow{2}*{w/o meta-path} & \multicolumn{3}{c}{Ours (meta-path)} \\
%     \multirow{2}*{Dataset}&\multirow{2}*{Base GNNs}& \multicolumn{2}{c|}{w/o meta-path} & \multicolumn{3}{c}{Ours (meta-path)} \\
%     %\hline
%     & & CE & MWNet & CE & SELAR & SELAR+Hint \\
%     %\toprule
%     \hline
%     \multirow{5}{*}{Last-FM} & GCN & 0.7898 & {0.7850}$^{*}$ & 0.8135 & \textbf{0.8163} & 0.8162 \\
%     & GAT & 0.8090 & 0.8100 & 0.8184 & 0.8319 & \textbf{0.8349} \\
%     & GIN & 0.7895 & 0.8081 & \textbf{0.8304} & 0.8211 & 0.8255 \\
%     & SGC & 0.7725 & 0.7759 & 0.7801 & 0.7803 & \textbf{0.7857} \\
%     \cline{2-7}
%     & Avg. Gain & 0 & +0.0046 & +0.0204 & +0.0222 & \textbf{+0.0253} \\
%     %\midrule
%     \hline
%     \multirow{5}{*}{Book-Crossing} & GCN & 0.6918 & 0.6967 & 0.6970 & \textbf{0.7081} & 0.7075 \\
%     & GAT & 0.6704 & 0.6759 & 0.7026 & 0.7136 & \textbf{0.7247} \\
%     & GIN & 0.6782 & 0.6968 & 0.7442 & 0.7554 & \textbf{0.7587} \\
%     & SGC & 0.6781 & {0.6732}$^{*}$ & 0.6933 & \textbf{0.7070} & 0.7039 \\
%     \cline{2-7}
%     & Avg. Gain & 0 & +0.0061 & +0.0297 & +0.0414 & \textbf{+0.0441}\\
%     %\toprule
%     \hline\hline
%   \end{tabular}
% \end{table}

% In Last-FM datasets, meta cross-validation works well compared to 1-fold for all models in our two frameworks, Selar and Selar with HintNet.
% Also, in node classification tasks, performance of all models enhance when we apply meta data with meta cross-validation methods.


==> Sections/meta-weight-net.tex <==
\textbf{Meta-Weight-Net}~\cite{han2018coteaching} is a meta-learning framework to train neural networks on noisy or skewed datasets.~\jw{For achieving this, Meta-Weight-Net learns an explicit sample-weight function to maximize its performance on an `ideal' test dataset called `meta-dataset', which contains noise-free or balanced data.} 
%Meta-Weight-Net learns an explicit sample-weight function to train a model on a noisy or skewed training dataset to maximize its performance on an `ideal' test dataset called `meta-dataset', which is a noise-free or balanced data. 
For example, assume that the target task is to learn a classifier $f(\xb; \wb)$, which has a good performance on a meta-dataset.
Meta-Weight-Net learns the sample-weight function $\mathcal{V}(\cdot;\Theta)$ parameterized by $\Theta$ so that 
a regular training with the sample-weights can find an optimal classifier $f(\xb;\wb^{\ast})$ for the meta-dataset.
The optimal parameters $\mathbf{w}^{\ast}$ can be  found by minimizing the following loss:  
% Then, given $N$ training samples, the training seeks the optimal model parameters $\mathbf{w}^{\ast}$ minimizing the weighted training loss given as 
\begin{equation}
\label{eq:mw_optimal}
\mathbf{w}^{\ast}(\Theta) = \underset{\mathbf{w}}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\Theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))\mathcal{L}_{i}^{train}(\mathbf{w}),
\end{equation} 
where $\Lc^{train}_i(\wb)  \triangleq \ell(y_i^{(train)}, f(x_i^{(train)};\wb))$ is the training loss for the $i_{th}$ sample, and $\mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))$ is the learned sample-weight.~\jw{$N$ denotes the training data size.}
% The weight is determined by parameters of weight function $\Theta$ and its input $L_{i}^{train}(\mathbf{w})$, which is $i$-th sample loss on classifier parameter $\mathbf{w}$.
% The optimal parameter of Meta-Weight-Net is obtained by equation:
% \begin{equation}
% \label{eq:mw_optimal}
% % \mathbf{w}^{\ast}(\theta) = \underset{w}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\theta)\mathcal{L}_{i}^{train}(\mathbf{w}),
% \mathbf{w}^{\ast}(\Theta) = \underset{\mathbf{w}}{\argmin} \ \mathcal{L}^{train}(\mathbf{w};\Theta) \triangleq \frac{1}{N}\sum_{i=1}^{N} \mathcal{V}(\mathcal{L}_{i}^{train}(\mathbf{w};\Theta))\mathcal{L}_{i}^{train}(\mathbf{w}),
% \end{equation} 
% where $N$ is number of train-data samples and $\mathbf{w}^{\ast}$ is the optimal classifier parameter. The hyper-parameter $\Theta$ is determined automatically in a meta-learning way. The optimal parameter $\Theta^{\ast}$ can be obtained by equation:
To optimize the sample-weights, the parameters $\Theta$ is optimized by 
\begin{equation}
\label{eq:mw_theta_optimal}
\Theta^{\ast} = \underset{\Theta}{\argmin} \ \mathcal{L}^{meta}(\mathbf{w}^{\ast}(\Theta)) \triangleq \frac{1}{M}\sum_{i=1}^{M} \mathcal{L}_{i}^{meta}(\mathbf{w}^{\ast}(\Theta)),
\end{equation}
where $M$ is the number of meta-data samples and $\mathcal{L}_{i}^{meta}(\mathbf{w}) = \ell(y_{i}^{(meta)}, f(x_{i}^{(meta)}, \mathbf{w}))$ is the validation loss on meta-data. 
This can be viewed as a form of meta-learning. 
Inspired by this work, we propose a meta-learning framework to learn a model with multiple auxiliary tasks to improve the performance of the primary task.
% We apply this concept to learn adaptively by learning auxiliary tasks. In section 3.2, we will show how we apply Meta-Weight-Net to train GNN task through multi meta-paths prediction tasks. 

==> Tables_tex/tab_CV_IMDB.tex <==
\begin{table}[h]
  \caption{Comparison between 1-fold and 3-fold as meta-data on \textbf{IMDB} datasets \jw{[결과되게 애매한데 뺄까요? 이테이블?]}}
  \label{tab:metacv_node}
  \centering
  \begin{tabular}{c|c|cc|cc}
    \toprule
     & & \multicolumn{2}{c}{SElAR} & \multicolumn{2}{c}{SELAR+Hint}\\
     
     Model &Vanilla &1-fold & 3-fold & 1-fold & 3-fold  \\
    \midrule
     GCN & 0.5809 & 0.5302 & \textbf{0.5994 }& 0.5663 &\textbf{ 0.5847}  \\
     GAT & 0.5587 & 0.6032 & \textbf{0.6126 }& \textbf{0.6017} & 0.6015   \\
     GIN & 0.5965 & \textbf{0.6140} & 0.5994 & \textbf{0.6015} & 0.5726  \\
     SGC & 0.5583 & 0.5829 & \textbf{0.6224 }& 0.5852 & \textbf{0.5906}  \\
    \bottomrule
  \end{tabular}
\end{table}

==> Tables_tex/tab_link_ablation.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table}[h]
  %\centering
  \caption{Link prediction performance ($AUC$-score) of GNNs}
  \footnotesize 
  \label{tab:add_link_prediction}
  \begin{tabular}{c@{ }c|rrr|rrr}
    \toprule
    %\hline
    Dataset & \shortstack{Base\\GNNs}  & Vanilla & \shortstack{Graph-MW\\ w/o mp} & \shortstack{Graph-MW\\ w/ mp} & SELAR &\shortstack{SELAR\\+Hint } &\shortstack{ Regularized\\SELAR+Hint }\\
    %\toprule
    \midrule
    \multirow{5}{*}{Last-FM} 
    & GCN & 0.7963 & 0.7889 & 0.7885 & 0.8296 & & \\
    & GAT & 0.8115 & 0.8115 & 0.8287 & 0.8307 & & \\
    & GIN & 0.8199 & 0.8217 & 0.8234 & 0.8361 & & \\
    & SGC & 0.7703 & 0.7766 & 0.7691 & 0.7827 & & \\
    \cmidrule{2-8}
    & Avg. Gain & - &  &  &  & & \\
    \midrule
    \multirow{5}{*}{\shortstack{Book\\Crossing}} 
    & GCN & 0.7039 & 0.7031 & 0.7110 & 0.7182 & &\\
    & GAT & 0.6891 & 0.6968 & 0.7075 & 0.7345 & &\\
    & GIN & 0.6979 & 0.7210 & 0.7338 & 0.7526 & &\\
    & SGC & 0.6860 & 0.6808 & 0.6792 & 0.6907 & &\\
    \cmidrule{2-8}
    & Avg. Gain & - & & & & & \\
    \toprule
  \end{tabular}
\end{table}

% \setlength{\tabcolsep}{8pt}
% \begin{table}[h]
%   %\centering
%   \caption{Link prediction performance ($AUC$-score) of GNNs}
%   \footnotesize 
%   \label{tab:add_link_prediction}
%   \begin{tabular}{c@{ }c|rrr|rr}
%     \toprule
%     %\hline
%     Dataset & Base GNNs & Vanilla & \shortstack{Graph-MW\\ w/o meta-path} & \shortstack{Graph-MW\\ w/ meta-path} & SELAR  &\shortstack{ Regularized\\SELAR+Hint }\\
%     %\toprule
%     \midrule
%     \multirow{5}{*}{Last-FM} & GCN & 0.7898 & 0.7850 & 0.7861 & 0.8163 & \textbf{0.8206}\\
%     & GAT & 0.8090 & 0.8100 & 0.8244 & 0.8319 & \textbf{0.8349}\\
%     & GIN & 0.7895 & 0.8081 & 0.8204 & 0.8211 & \textbf{0.8262}\\
%     & SGC & 0.7725 & 0.7759 & 0.7400 & 0.7803 & \textbf{0.8029} \\
%     \cmidrule{2-7}
%     & Avg. Gain & - & +0.0046 & +0.0025 & +0.0222 & \\
%     \midrule
%     \multirow{5}{*}{Book-Crossing} & GCN & 0.6918 & 0.6967 & 0.7047 & 0.7081 & \textbf{0.7109}\\
%     & GAT & 0.6704 & 0.6759 & 0.7075 & 0.7136 & \textbf{0.7290}\\
%     & GIN & 0.6782 & 0.6968 & 0.7543 & 0.7554 & \textbf{0.7602}\\
%     & SGC & 0.6781 & 0.6732 & 0.7038 & 0.7070 & \textbf{0.7088}\\
%     \cmidrule{2-7}
%     & Avg. Gain & - & +0.0061 & +0.0380 & +0.0414 & \\
%     \toprule
%   \end{tabular}
% \end{table}


==> Tables_tex/tab_node_ablation.tex <==
\setlength{\tabcolsep}{8pt}
\begin{table}[ht]
  \centering
  \caption{Node classification performance ($F1$-score) of GNNs}
  \footnotesize 
  \label{tab:abb_node_classification}
  \begin{tabular}{cc|rr|rrr}
    \toprule
    Dataset & Base GNNs & Vanilla & Graph-MW & SELAR & SELAR+Hint & \shortstack{ Regularized\\SELAR+Hint }\\
    %\hline
    %\toprule
    \midrule
    \multirow{5}{*}{ACM} & GCN & 0.9034 & 0.9061 & 0.9147 & \textbf{0.9160} & 0.9058\\
    & GAT & 0.9179 & 0.9183 & \textbf{0.9198} & 0.9188 & 0.9095\\
    & GIN & 0.9060 & 0.9100 & 0.9076 & 0.9135 & \textbf{0.9191}\\
    & SGC & 0.9138 & 0.9128 & 0.9158 & \textbf{0.9171} & 0.9124\\
    \cmidrule{2-7}
    & Avg. Gain & - & +0.0015 & +0.0030 & \textbf{+0.0060} & \\
    \midrule
    \multirow{5}{*}{IMDB} & GCN & 0.5826 & 0.5812 & 0.6072 & 0.5970 & \textbf{0.6119}\\
    & GAT & 0.5587 & 0.5697 & \textbf{0.6197} & 0.6017 & 0.5942\\
    & GIN & 0.5965 & 0.5972 & \textbf{0.5994} & 0.5974 & 0.5885\\
    & SGC & 0.5675 & 0.6132 & \textbf{0.6147} & 0.5957 & 0.6088\\
    \cmidrule{2-7}
    & Avg. Gain & - & +0.0140 & \textbf{+0.0340} & +0.0217 & \\
    \bottomrule
  \end{tabular}
\end{table}

